NeuDep: Neural Binary Memory Dependence Analysis

Determining whether multiple instructions can access the same memory location is a critical task in binary analysis. It is challenging as statically computing precise alias information is undecidable in theory. The problem aggravates at the binary level due to the presence of compiler optimizations and the absence of symbols and types. Existing approaches either produce significant spurious dependencies due to conservative analysis or scale poorly to complex binaries. We present a new machine-learning-based approach to predict memory dependencies by exploiting the model's learned knowledge about how binary programs execute. Our approach features (i) a self-supervised procedure that pretrains a neural net to reason over binary code and its dynamic value flows through memory addresses, followed by (ii) supervised finetuning to infer the memory dependencies statically. To facilitate efficient learning, we develop dedicated neural architectures to encode the heterogeneous inputs (i.e., code, data values, and memory addresses from traces) with specific modules and fuse them with a composition learning strategy. We implement our approach in NeuDep and evaluate it on 41 popular software projects compiled by 2 compilers, 4 optimizations, and 4 obfuscation passes. We demonstrate that NeuDep is more precise (1.5x) and faster (3.5x) than the current state-of-the-art. Extensive probing studies on security-critical reverse engineering tasks suggest that NeuDep understands memory access patterns, learns function signatures, and is able to match indirect calls. All these tasks either assist or benefit from inferring memory dependencies. Notably, NeuDep also outperforms the current state-of-the-art on these tasks.

==> case.tex <==
\section{Case Studies}
\label{sec:case}

\subsection{Probing the Learned Knowledge}
\label{subsec:probing}

\vspace{.1cm}\noindent\textbf{Learning function signature.} 
Recovering function signatures has traditionally been a critical intermediate step in the process of predicting indirect calls. Therefore, in order to validate $\sys's$  end-to-end call prediction performance, asking $\sys$ to predict function signatures can serve as a useful probing task. We follow EKLAVYA and implement a total of 8 different finetuning tasks in this domain. Tasks 1-4 ask the model to recover a function's argument count and the types of the 1st, 2nd, and 3rd arguments from the callsite within the caller. Tasks 5-8 ask the model to predict the same labels, but based on the callee body.

Formally, the input to each callee task is a function $F_{callee}$. The input to each caller task is a pair $(F_{caller}, L)$, where $L$ is a list that contains the indices of the callsite instructions within $F_{caller}$.

We finetune $\sys$ on the dataset provided by EKLAVYA for 100 epochs with a batch size of 32, and evaluate the performance of each finetuning head on a hold-out test set, also taken from the same dataset. We compare our results across multiple optimization levels with EKLAVYA. EKLAVYA treats function signature recovery as a collection of multiple independent classification tasks, one for the argument count and one for the type of each argument position. EKLAVYA also reports the prediction accuracy (as opposed to F1 score). We therefore also evaluate $\sys$'s accuracy on each task, defined as the number of correctly lables divded by the total sample size.

$\sys$ outperforms EKLAVYA across every task and every optimization level, achieving x\% higher accuracy on average. Most notably, $\sys$'s performance remains robust across every task and optimization level, while EKLAVYA has a clear drop for higher optimization levels and higher argument positions. We conjecture that this difference in robustness can be explained by the difference in approach between the two models. Whereas $\sys$ is trained on execution traces, which are in some sense invariant to increased optimization, EKLAVYA only leverages knowledge of static instruction tokens, which become harder to decipher as optimization increases. 

\vspace{.1cm}\noindent\textbf{Caller-callee matching via predicted function signatures.}
To further demonstrate the robustness of $\sys$'s end-to-end indirect call prediction, we show evidence that $\sys$'s ability to predict function signatures can be directly leveraged to perform caller-callee matching. We define a deterministic function $M: \mapsto \{0,1\}$

\vspace{.1cm}\noindent\textbf{Predicting execution states.}

\vspace{.1cm}\noindent\textbf{Learned representation of numeric values.}

\subsection{Malware Behavioral Analysis}



==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Unlike traditional approaches based on abstract interpretation~\cite{debray1998alias, cifuentes1997intraprocedural, brumley2006alias, reps2008improved, balakrishnan2004analyzing, balakrishnan2010wysinwyx} that feature conservativeness, \sys does not guarantee soundness. 
As shown in Section~\ref{sec:eval}, the key advantage of \sys is that it is much more \emph{precise} and \emph{scalable} than existing tools.

\vspace{.1cm}
\noindent\textbf{Precision.}
The major obstacle preventing VSA from being practical is that it reports substantial bogus dependencies~\cite{zhang2019bda, guo2019vsa}.
In practice, a precise but unsound detection of memory dependencies is useful for many applications~\cite{heo2017machine}, such as reverse execution for debugging crashes~\cite{mu2019renn, cui2018rept}, inferring indirect calls~\cite{farkhani2018effectiveness}, malware analysis~\cite{cozzi2018understanding}, and decompilation~\cite{david2020neural}.
Recent human studies also show that precise memory dependence analysis significantly benefit developers during manual code inspection~\cite{matzen2021effects}.

\vspace{.1cm}
\noindent\textbf{Scalability.}
Efficiently uncovering large number of memory dependencies is desirable for many applications.
For example, by using \sys, we can build the program dependence graphs of a large number of binary functions. 
Such a dependence graph is often used to match semantically similar functions~\cite{xu2017neural} and recovering debugging information~\cite{david2020neural, he2018debin}.
% We envision exciting future works by applying \sys for many other downstream applications.

\vspace{.1cm}
\noindent\textbf{Reasoning compositionality of instructions.} Multi-hop

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}

Statically inferring memory dependencies requires the model to understand the behavior of instructions and reason about the potential value flows. 
A typical setup of supervised learning would directly learn the mapping from static instructions to their dependencies. 
We use the following motivating examples to demonstrate an ML model trained this way tends to rely on spurious statistical code patterns without understanding the instructions' semantics.
% As opposed to the common belief that the code semantics emerge from big code~\cite{allamanis2018survey, raychev2015predicting, hindle2016naturalness}, our key observation is that the semantics of instructions, unlike regular text, is \emph{grounded} in its execution behavior, manifested in its execution traces~\cite{heule2016stratified, nye2020representing}.
% \bray{This motivation is a bit confusing----are you trying to motivate pretraining or training with traces? I think bothe are important. We should not assume readers know what pretraining is.}

\begin{example}
\label{ex:deepvsa_fail}
Figure~\ref{fig:task_definition} shows that two instructions \code{mov rdi,[rax+0x8]} and \code{mov [rbp+rbx],rdi} access the same memory location but via different addressing registers.
To detect the dependency, the model needs to first understand that the behavior of \code{mov}: both line 1 ($I_1$) and line 4 ($I_4$) set \code{rax} and \code{rbx} to the same value.
It then needs to understand \code{xor} in line 5 sets \code{rbp} to 0, and \code{add} in line 6 performs addition and sets \code{rbp} to \texttt{0x8}. 
Finally, the model needs to compose these facts and concludes that \code{rax+0x8} is equivalent to \code{rbp+rbx} in such a context.
However, we find that when running the ML models trained only on static code for this task~\cite{li2021palmtree, guo2019vsa}, they predict that line 2 accesses a heap object, but line 7 writes to stack, possibly because they observe the pattern that the stack base pointer \code{rbp} is used at line 7, and \code{rax}, which often stores the return value of \code{malloc}, is used at line 2.
As the trained ML model is used to instantiate the value set used by VSA~\cite{guo2019vsa}, this misprediction thus leads to a false negative by flagging two instructions as accessing non-overlapping memory regions.
\end{example}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{./figs/task_definition.pdf}

\caption{Motivating example of predicting memory dependencies in the function \texttt{ngx\_init\_setproctitle} from \texttt{nginx-1.21.1}. 
% We highlight the dependent instructions pair in \colorbox{lightblue}{blue} and that without in \colorbox{lightred}{red}.
$I_2$ and $I_7$ access the same heap variable (in \colorbox{lightblue}{blue}); $I_3$ and $I_8$ access the two \emph{different} global variables (in \colorbox{lightred}{red}). 
We find existing ML-based approaches~\bray{is it static only} fail to detect $I_2$ and $I_7$ are dependent by predicting they access to different memory regions, and cannot distinguish the memory accessed by $I_3$ and $I_8$ due to the prediction granularity.}
\bray{Change I to Instruction, 1,2,3, as I1, I2, etc.}

\label{fig:task_definition}
\end{figure}

The above observation underscores the importance of encoding the knowledge of instructions' behavior as part of the ML model.
% The typical way of achieving this is via designing input features encoding code behaviors as a compact representation (\ie category) by domain expert.
% Such a method is known requiring nontrivial manual effort, \ie covering the complete instruction set.
% Moreover, it is unclear how the model can learn the compositions of the extracted features to generalize to different 
In this paper, we automate the encoding process by pretraining the model to interpret and synthesize assembly code by employing \emph{masking} on diverse instructions and their execution traces.
We then train the model to predict what is masked based on the instructions and its execution traces not masked.
To minimize the prediction losses, the model needs to encode the side effect of each instruction in computing value flows as part of their embeddings.

Depending on where the masks are applied, each data sample requires making sense of different instructions to make the prediction.
We use Table~\ref{tab:example} to demonstrate how the location of applied masks affects the learned instruction semantics.

\begin{example}[{\em Interpreting} Bitwise Ops]
\label{ex:interpret_bitwise}
The first row in Table~\ref{tab:example} shows an example when the output of \code{xor} is masked for the instruction \code{xor rax,rbx}.
Observing \code{rax}=\texttt{0x2} and \code{rax}=\texttt{0x7} before running the instruction, the model needs to understand the operational semantics of \code{xor} to predict \code{rax}=\texttt{0x5} after executing this instruction.
Moreover, it trains the model to learn the syntax of x86-64 instruction set, where \code{xor} updates the first operand in place.
\end{example}

\begin{example}[{\em Synthesizing} Arithmetic Ops]
The second row in Table~\ref{tab:example} shows that the mnemonic \code{add} is masked in \code{add rbp,0x8} (we use \code{const} to denote the constant \code{0x8} and put its value in the trace).
To predict the masked \code{add} (out of the candidates like \code{sub}, \code{mov}, etc.), the model needs to associate \code{add} to the behavior that increments the value of its first operand by that of its second operand.
\end{example}

\begin{example}[Reverse {\em Interpreting} Arithmetic Ops]
The third row in Table~\ref{tab:example} shows an example when the input (the value of \code{rcx}) of \code{sub rcx,rdx} is masked.
To predict the masked input value \texttt{0x9}, the model needs to interpret the reverse execution behavior of \code{sub} given its output \texttt{0x8} and the value of its second operand \texttt{0x1}.
Such a task benefits the model when it needs to back-propagate values, and trace reverse value flows to infer memory dependencies.
\end{example}

\begin{example}[{\em Interpreting} Compositions of Memory Ops]
\label{ex:compose}
The last row in Table~\ref{tab:example} shows when executing more than one instructions and the output (the value of \code{rsi}) of~\code{mov rsi,[rsp]} is masked.
To predict the masked value \texttt{0x6}, the model needs to first interpret \code{push} and understand its side effect: decrements the stack pointer \code{rsp} by 8 bytes and store the value of \code{rdi} (\texttt{0x6}) on stack referenced by \code{rsp}.
The model then needs to interpret \code{mov} and understands it assigns the value from its second operand to the first operand.
Finally, by combining the fact that \code{push} stores \texttt{0x6} at location \texttt{0x0} and \code{mov} loads the value stored at \texttt{0x0} and assigns to \code{rsi}, the model can infer the masked value to be \texttt{0x6}.
\end{example}

\input{tables/examples}
